Span-core Decomposition for Temporal Networks: Algorithms and Applications

When analyzing temporal networks, a fundamental task is the identification of dense structures (i.e., groups of vertices that exhibit a large number of links), together with their temporal span (i.e., the period of time for which the high density holds). In this paper we tackle this task by introducing a notion of temporal core decomposition where each core is associated with two quantities, its coreness, which quantifies how densely it is connected, and its span, which is a temporal interval: we call such cores \emph{span-cores}. For a temporal network defined on a discrete temporal domain $T$, the total number of time intervals included in $T$ is quadratic in $|T|$, so that the total number of span-cores is potentially quadratic in $|T|$ as well. Our first main contribution is an algorithm that, by exploiting containment properties among span-cores, computes all the span-cores efficiently. Then, we focus on the problem of finding only the \emph{maximal span-cores}, i.e., span-cores that are not dominated by any other span-core by both their coreness property and their span. We devise a very efficient algorithm that exploits theoretical findings on the maximality condition to directly extract the maximal ones without computing all span-cores. Finally, as a third contribution, we introduce the problem of \emph{temporal community search}, where a set of query vertices is given as input, and the goal is to find a set of densely-connected subgraphs containing the query vertices and covering the whole underlying temporal domain $T$. We derive a connection between this problem and the problem of finding (maximal) span-cores. Based on this connection, we show how temporal community search can be solved in polynomial-time via dynamic programming, and how the maximal span-cores can be profitably exploited to significantly speed-up the basic algorithm.

==> figures/spancoresVSmlcores.tex <==

\begin{tikzpicture} [scale=0.20, every node/.style={circle, draw, scale=0.65}]
	% \node (name) at (horizontal,vertical) {label}; --> (0,0) is the lower left corner
	\node (A) at (0,10) {\textsf{A}};
	\node (B) at (10,10) {B};	
	\node (C) at (20,10) {C};
	\node (D) at (0,0) {D};
	\node (E) at (10,0) {E};
	\node (F) at (20,0) {F};
	
	\draw (A) edge (B);
	\draw (A) edge (D);
	%\draw (A) edge (E);
	\draw (B) edge (C);
	%\draw (B) edge (D);
	\draw (B) edge (E);
	%\draw (B) edge (F);
	\draw (D) edge (E);
	%\draw (E) edge (F);
	
	\draw [dashed, bend left=10] (A) edge (B);
	\draw [dashed] (A) edge (E);
	%\draw [dashed, bend left=10] (B) edge (C);
	\draw [dashed] (B) edge (D);
	%\draw [dashed, bend left=10] (B) edge (E);
	%\draw [dashed, bend left=10] (B) edge (F);
	\draw [dotted] (C) edge (E);
	\draw [dotted] (C) edge (F);
	\draw [dashed, bend right=10] (D) edge (E);
	\draw [dashed] (E) edge (F);
\end{tikzpicture}

==> maximal_cs.tex <==


\begin{algorithm}[t]
\DontPrintSemicolon
\newcommand\commentfont[1]{\small\ttfamily{#1}}
\SetCommentSty{commentfont}

\KwIn{A temporal graph $G = (V,E,T)$, a set $Q \subseteq V$ of query vertices, an integer $h \in \mathbb{N}^+$.}
%\KwOut{A set $\{\Delta_i\}_{i=1}^h$ of temporal intervals such that $\bigcup_{i=1}^h \Delta_i = T$.}
\KwOut{A set $\{\langle S_i, \Delta_i \rangle\}_{i=1}^h$, where $Q \subseteq S_i \subseteq V$, $\forall 1 \leq i \leq h$, and $\{\Delta_i\}_{i=1}^h$ is a partition of $T$.}

\tcc{Identification of $T^*$}

Compute the set $\mathbf{C}_M(Q)$ of $Q$-constrained maximal \spancores of $G$\;
$\mathbf{D} \leftarrow \{\Delta \sqsubseteq T \mid C_{k,\Delta} \in \mathbf{C}_M(Q) \}$ \label{line:maximaltemporalcs:cd}\;
%$T_{\mathbf{D}} \leftarrow \{ t \mid \exists \Delta \in \mathbf{D} : t \in \Delta \}$\;
$T_{\mathbf{D}} \leftarrow \bigcup_{\Delta \in \mathbf{D}} \Delta$; \ $T_{\mathbf{D}}^+ \leftarrow \{\min\{t_e \!+\! 1, t_{max}\} \mid [t_s,t_e] \in \mathbf{D}\}$; \ $T_{\mathbf{D}}^- \leftarrow \{\max\{t_s \!-\! 1, 0\} \mid [t_s,t_e] \in \mathbf{D}\}$\;
$T^* \leftarrow T_{\mathbf{D}} \ \cup \ T_{\mathbf{D}}^+ \ \cup \ T_{\mathbf{D}}^- \ \cup \ \{0, 1, \ldots, h-1\} \ \cup \ \{t_{max}\}$\;


\tcc{Initialization}
$\mathbf{M} \leftarrow \{$row index$: t, \forall t \in T^*\}$\;
$\mathbf{P} \gets$ an empty  $(|T^*| \times h)$-dimensional matrix \tcp*{Penalty matrix}
$\mathbf{R} \gets$ an empty $(|T^*| \times h)$-dimensional matrix \tcp*{Reconstruction matrix}


\ForAll{$r \in \mathbf{M}$}
{
	$\mathbf{P}[r,0] \gets -v^*_{Q, [0,\mathbf{M}[r]]}$\;
	$\mathbf{R}[r,0] \gets 0$\;
}

\tcc{Dynamic-programming step}
\ForAll{$r \in \mathbf{M}$}
{
	\ForAll{$i \in [1, h)$}
	{
		$\mathbf{P}[r,i] \gets \min_{\ell \in [0,r]} \mathbf{P}[\ell,i-1] - v^*_{Q, [\mathbf{M}[\ell+1],\mathbf{M}[r]]}$\;
		$\mathbf{R}[r,i] \gets \operatorname{argmin}_{\ell \in [0,r]} \mathbf{P}[\ell,i-1] - v^*_{Q, [\mathbf{M}[\ell+1],\mathbf{M}[r]]}$\;
	}
}

\tcc{Reconstruction of the solution}
$ub \gets |T^*| - 1$\;
\ForAll{$i \in (h, 0]$}
{
	$lb \gets \mathbf{R}[ub,i]$\;
	$\Delta_i \gets [\mathbf{M}[lb], \mathbf{M}[ub]]$\;
	$ub \gets lb - 1$\;
}
\ForAll{$i \in (h, 0]$}
{
	$S_i \gets C^*_{Q, \Delta_i}$
}

\caption{\mcs}\label{alg:maximaltemporalcs}
\end{algorithm}

==> naive_cs.tex <==


\begin{algorithm}[t]
\DontPrintSemicolon
\newcommand\commentfont[1]{\small\ttfamily{#1}}
\SetCommentSty{commentfont}

\KwIn{A temporal graph $G = (V,E,T)$, a set $Q \subseteq V$ of query vertices, an integer $h \in \mathbb{N}^+$.}
\KwOut{A set $\{\langle S_i, \Delta_i \rangle\}_{i=1}^h$, where $Q \subseteq S_i \subseteq V$, $\forall 1 \leq i \leq h$, and $\{\Delta_i\}_{i=1}^h$ is a partition of $T$.}



\vspace{1mm}
\tcc{Initialization}
Compute $v^*_{Q,\Delta}$ and $C^*_{Q,\Delta}$, $\forall \Delta \sqsubseteq T$, via $Q$-constrained \spancore decomposition\;
$\mathbf{P} \gets$ an empty  $(|T| \times h)$-dimensional matrix \tcp*{Penalty matrix}
$\mathbf{R} \gets$ an empty $(|T| \times h)$-dimensional matrix \tcp*{Reconstruction matrix}
\ForAll{$t \in T$}
{
	$\mathbf{P}[t,0] \gets -v^*_{Q, [0,t]}$\;
	$\mathbf{R}[t,0] \gets 0$\;
}

\tcc{Dynamic-programming step}
\ForAll{$t \in T$}
{
	\ForAll{$i \in [1, h)$}
	{
		$\mathbf{P}[t,i] \gets \min_{\ell \in [0, t]} \mathbf{P}[\ell,i-1] - v^*_{Q,[\ell+1,t]}$\;
		$\mathbf{R}[t,i] \gets \operatorname{argmin}_{\ell \in [0, t]} \mathbf{P}[\ell,i-1] - v^*_{Q,[\ell+1,t]}$\;
	}
}

\tcc{Reconstruction of the solution}
$ub \gets t_{max}$\;
\ForAll{$i \in (h, 0]$}
{
	$lb \gets \mathbf{R}[ub,i]$\;
	$\Delta_i \gets [lb, ub]$\;
	$ub \gets lb - 1$\;
}
\ForAll{$i \in (h, 0]$}
{
	$S_i \gets C^*_{Q, \Delta_i}$
}

\caption{\cs}\label{alg:temporalcsnaive}
\end{algorithm}

==> pseudocodes/baseline.tex <==


\begin{algorithm}[t]
	\caption{\baseline}
	\begin{algorithmic}[1] \label{alg:baseline}
		\REQUIRE A temporal graph $G=(V,T,\tau)$.
		\ENSURE The set $\coresset$ of all \spancores of $G$.

		\STATE  $\coresset \leftarrow \emptyset$
		
		\vspacealg
		
		\FORALL{$\Delta \sqsubseteq T$}
			\STATE $E_\Delta  \leftarrow \bigcap_{t \in \Delta} E_t$
			%\STATE $\coresset \leftarrow \coresset 	\ \cup$ \deltacores $(G, V, \Delta)$\hfill\COMMENT{Algorithm~\ref{alg:deltacores}}
			\STATE $\coresset \leftarrow \coresset 	\ \cup$ \textsf{core-decomposition}$(V,E_{\Delta})$ \label{line:baseline:decomposition}
		\ENDFOR
	\end{algorithmic}
\end{algorithm}


==> pseudocodes/inner_most_core.tex <==


\begin{algorithm}[t]
	\caption{\innermost}
	\begin{algorithmic}[1] \label{alg:imcore}
		\REQUIRE A simple graph $G=(V,E)$ and a subset of vertices $S \subseteq V$.
		\ENSURE The maximal core $\imcore$ of $G$ and its minimum degree $\imk$.
		
		\STATE $\imcore \leftarrow \emptyset$, $\imk \leftarrow 0$
		\STATE $d \leftarrow \emptyset$, $\mathcal{D} \leftarrow [\emptyset, \ldots, \emptyset]$
		
		\vspacealg		
		
		\FORALL{$u \in S$}
			\STATE $d[u] \leftarrow \deg(S,u)$
			\STATE $\mathcal{D}[d[u]] \leftarrow \mathcal{D}[d[u]] \cup \{u\}$
		\ENDFOR
		
		\vspacealg
		
		\FORALL{$k \in [0,|\mathcal{D}|)$}
			\WHILE{$\mathcal{D}[k] \neq \emptyset$}
				\STATE pick and remove a vertex $u$ from $\mathcal{D}[k]$
				\STATE $S \leftarrow S \setminus \{u\}$
				
				\vspacealg
				
				\FORALL{$v \in S \mid (u,v) \in E, d[v] > k$}
					\STATE $\mathcal{D}[d[v]] \leftarrow \mathcal{D}[d[v]] \setminus \{v\}$
					\STATE $\mathcal{D}[d[v] - 1] \leftarrow \mathcal{D}[d[v] - 1] \cup \{v\}$
					\STATE $d[v] \leftarrow d[v] - 1$
				\ENDFOR
			\ENDWHILE
			
			\vspacealg
			
			\STATE $\imcore \leftarrow S$, $\imk \leftarrow k+1$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

==> pseudocodes/subroutine.tex <==


\begin{algorithm}[t]
	\caption{\deltacores}
	\begin{algorithmic}[1] \label{alg:deltacores}
		\REQUIRE A temporal graph $G=(V,E,T,\tau)$, a subset of vertices $S \subseteq V$, and a temporal interval $\Delta \sqsubseteq T$.
		\ENSURE The set $\coressetessedelta$ of all temporal cores of $G[S,\Delta]$.
		
		\vspacealg
		
		\STATE $\coressetessedelta \leftarrow \emptyset$
		\STATE $\delta \leftarrow \emptyset$, $\mathcal{D} \leftarrow [\emptyset, \ldots, \emptyset]$

		\vspacealg
		
		\FORALL{$u \in S$} \label{line:deltacores:ciclestart}
			\STATE $\delta[u] \leftarrow \tdeg_\Delta(S,u)$ \label{line:deltacores:degree}
			\STATE $\mathcal{D}[\delta[u]] \leftarrow \mathcal{D}[\delta[u]] \cup \{u\}$
		\ENDFOR \label{line:deltacores:cicleend}
		
		\vspacealg
		
		\FORALL{$k \in [0,|\mathcal{D}|)$}
			\WHILE{$\mathcal{D}[k] \neq \emptyset$}
				\STATE pick and remove a vertex $u$ from $\mathcal{D}[k]$
				\STATE $S \leftarrow S \setminus \{u\}$
				
				\vspacealg
				
				\FORALL{$v \in S \mid (u,v) \in E[\Delta, S], \delta[v] > k$}
					\STATE $\mathcal{D}[\delta[v]] \leftarrow \mathcal{D}[\delta[v]] \setminus \{v\}$
					\STATE $\mathcal{D}[\delta[v] - 1] \leftarrow \mathcal{D}[\delta[v] - 1] \cup \{v\}$
					\STATE $\delta[v] \leftarrow \delta[v] - 1$
				\ENDFOR
			\ENDWHILE
			
			\vspacealg
			
			\STATE $\coressetessedelta \leftarrow \coressetessedelta \cup \{S\}$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}
